Recent results from the cosmic ray program of the NA61/SHINE experiment

NA61/SHINE is a fixed target experiment designed to study hadron-proton, hadron-nucleus and nucleus-nucleus interactions at the CERN Super-Proton-Synchrotron. In this paper we summarize the results from pion-carbon collisions recorded at beam momenta of 158 and 350 GeV/c. Hadron production measurements in this type of interactions is of fundamental importance for the understanding of the muon production in extensive air showers. In particular, production of (anti)baryons and $\rho^0$ are mechanisms responsible for increasing the number of muons which reaches the ground. The underestimation of the (anti)baryons or $\rho^0$ production rates in current hadronic interaction models could be one of the sources of the excess of muons observed by cosmic ray experiments. The results on the production spectra of $\pi^{\pm}$, K$^{\pm}$, p, $\bar{\text{p}}$, $\Lambda$, $\bar{\Lambda}$, K$^{0}_\text{S}$, $\rho^0$, $\omega$ and K$^{0*}$ are presented, as well as their comparison to predictions of hadronic interaction models currently used in air shower simulations.

==> BeamerUtil.tex <==
%%LOCAL COLORS
\definecolor{ThisBlue}{RGB}{50,50,168}
\definecolor{ThisRed}{RGB}{225,0,0}
\definecolor{ThisGray}{RGB}{150,150,150}


%%FUNCTIONS
\def\Put(#1,#2)#3{\leavevmode\makebox(0,0){\put(#1,#2){#3}}}

\newcommand{\hsp}[1]{\hspace*{#1cm}}
\newcommand{\vsp}[1]{\vspace*{#1cm}}

\newcommand{\reference}[1]{\textcolor{ThisGray}{#1}}
\newcommand{\arxiv}[1]{\href{https://arxiv.org/abs/#1}{\texttt{arXiv:#1}}}


%%BULLETS
\newcommand{\myarrow}{\textcolor{ThisRed}{\raisebox{0.4ex}[-0.4ex]{\tiny$\blacktriangleright$\xspace}}}
\newcommand{\mybullet}{\textcolor{ThisBlue}{\footnotesize $\bullet$}\xspace}  


%%ENVIROMENTS
\newcommand{\bc}{\begin{center}}
\newcommand{\ec}{\end{center}}
\newcommand{\bcols}{\begin{columns}}
\newcommand{\ecols}{\end{columns}}
\newcommand{\bcol}{\begin{column}}
\newcommand{\ecol}{\end{column}}
\newcommand{\bop}{\begin{overpic}}
\newcommand{\eop}{\end{overpic}}
\newcommand{\bbe}{\begin{equation*}}
\newcommand{\eee}{\end{equation*}}
\newcommand{\btikz}{\begin{tikzpicture}}
\newcommand{\etikz}{\end{tikzpicture}}

\newcommand{\bbox}[1]{\begin{tcolorbox}[colframe=#1,colback=white,left=0.2pt,right=0.2pt,top=0.5pt,bottom=0.5pt]}
\newcommand{\ebox}{\end{tcolorbox}}

